Exploiting Unstructured Sparsity in Fully Homomorphic Encrypted DNNs

The deployment of deep neural networks (DNNs) in privacy-sensitive environments is constrained by computational overheads in fully homomorphic encryption (FHE). This paper explores unstructured sparsity in FHE matrix multiplication schemes as a means of reducing this burden while maintaining model accuracy requirements. We demonstrate that sparsity can be exploited in arbitrary matrix multiplication, providing runtime benefits compared to a baseline naive algorithm at all sparsity levels. This is a notable departure from the plaintext domain, where there is a trade-off between sparsity and the overhead of the sparse multiplication algorithm. In addition, we propose three sparse multiplication schemes in FHE based on common plaintext sparse encodings. We demonstrate the performance gain is scheme-invariant; however, some sparse schemes vastly reduce the memory storage requirements of the encrypted matrix at high sparsity values. Our proposed sparse schemes yield an average performance gain of 2.5x at 50% unstructured sparsity, with our multi-threading scheme providing a 32.5x performance increase over the equivalent single-threaded sparse computation when utilizing 64 cores.

==> alg/algorithm_orig.tex <==

\SetAlgoNoLine
\begin{algorithm}[h]
\footnotesize
\KwIn{Encrypted list of chunks $A$ and $B$ representing respective matrices and corresponding matrix information $LHS$ and $RHS$.}
\KwOut{Encrypted matrix product, stored in list of chunks, $R$}
    % \Begin{
        \For{$row \text{ in } |result_{rows}|$}{
            \For{$col \text{ in } |result_{cols}|$}{
                \For{$k \text{ in } |LHS_{cols}|$}{
                    $\cdots$ \tcp*{Load chunks and calculate value offsets within chunks}
                    
                    \BlankLine
                
                    $a \longleftarrow fhe\_rotate(A_{chunk}, A_{offset})$ \tcp*{Load LHS value into slot zero}
                    $b \longleftarrow fhe\_rotate(B_{chunk}, B_{offset})$  \tcp*{Load RHS value into slot zero}
                    $a \longleftarrow a \cdot b$ \tcp*{Multiply operands}
                    $a \longleftarrow fhe\_relin(a)$ \tcp*{Re-linearise}
                    $a \longleftarrow fhe\_rescale(a)$ \tcp*{Switch to next modulus and rescale}
        
                    \BlankLine
        
                    $a \longleftarrow a \cdot zero\_mask$ \tcp*{Multiply with slot zero mask}
                    $a \longleftarrow fhe\_relin(a)$ \tcp*{Re-linearise}
                    $a \longleftarrow fhe\_rescale(a)$ \tcp*{Switch to next modulus and rescale}
        
                    \BlankLine
        
                    $a \longleftarrow fhe\_rotate(a, -R_{offset})$ \tcp*{Rotate product to result offset slot}
                    $R_{chunk} \longleftarrow fhe\_add(R_{chunk}, a)$ \tcp*{Add to result chunk}
                }
            }
        }
    % }    
    \caption{Algorithm for naive dense matrix multiplication in FHE.}
    \label{alg:dense-fhe-matmul}
\end{algorithm}
